Systems Modeling for novice engineers to comprehend software products better

One of the key challenges for a novice engineer in a product company is to comprehend the product sufficiently and quickly. It can take anywhere from six months to several years for them to attain mastery but they need to start delivering results much before. SaaS (Software-as-a-Service) products have sophisticated system architecture which adds to the time and effort of understanding them. On the other hand, time available to new hires for product understanding continues to be short and getting shorter, given the pressure to deliver more in less time. Constructivist theory views learning as a personal process in which the learner constructs new knowledge for themselves. Building and refining a mental model is the key way in which they learn, similar to how the brain operates. This paper presents an approach to improve system comprehension process by using a system model that a) acts as a transitional object to aid and refine the mental model of the learner, and b) captures the current understanding of the dynamics of the software system in a way that can be reasoned with and simulated. We have adapted discrete systems modeling techniques and used a transition system as a lightweight modeling language. Such a model can be used by novice engineers during their product ramp-up phase to build a model of the software system that captures their knowledge of the system and aid their mental model. The paper also presents a learning approach in which the learners create and refine these models iteratively using the available and newly uncovered knowledge about the software system. We hypothesize that by leveraging this modeling language and approach, novice engineers can reduce the time it takes them to achieve desired proficiency level of system comprehension. This paper presents early ideas on this language and approach.

==> c-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This paper presents an idea for helping novice engineers at SaaS product companies comprehend software systems better, by using a personal modeling language and approach while ramping up on the product. Given the complexity of SaaS products, the need for the engineers to understand the entire system behavior, and lack of time to ramp-up, it is important that any such language should be easy to learn and use and compliment the existing processes and resources. We present a transition systems based modeling language, and an iterative model refinement approach to aid software system comprehension for novice engineers. We expect that it will be easy for the novice engineers to learn and use. While this is still an initial idea, based on a few classes delivered to students and workshops conducted for novice engineers, we feel this can significantly help novice engineers when they ramp-up on the product. 
